Three-Dimensional Euler Fluid Code for Fusion Fuel Ignition and Burning

The document describes a numerical algorithm to simulate plasmas and fluids in the 3 dimensional space by the Euler method, in which the spatial meshes are fixed to the space. The plasmas and fluids move through the spacial Euler mesh boundary. The Euler method can represent a large deformation of the plasmas and fluids. On the other hand, when the plasmas or fluids are compressed to a high density, the spatial resolution should be ensured to describe the density change precisely. The present 3D Euler code is developed to simulate a nuclear fusion fuel ignition and burning. Therefore, the 3D Euler code includes the DT fuel reactions, the alpha particle diffusion, the alpha particle deposition to heat the DT fuel and the DT fuel depletion by the DT reactions, as well as the thermal energy diffusion based on the three-temperature compressible fluid model.

==> figure.tex <==
\begin{figure}[htbp]
\begin{center}
\includegraphics[width=130mm]{figure/figure1} \\ 
\vspace{3zh}
\includegraphics[width=120mm]{figure/figure2} \\
\end{center}
\end{figure}
\newpage
\begin{figure}[htbp]
\includegraphics[width=130mm]{figure/figure3} \\
\end{figure}

==> title.tex <==
%\documentclass[dvipdfmx]{jarticle}
%\usepackage[left=30mm,right=30mm,top=35mm,bottom=35mm]{geometry}

%\begin{document}
	\begin{center}
		{\bf 3-Dimensional Euler Code for Fusion Fuel ignition and Burning}  \\
		\vspace{10truept}
		Hiroki Nakamura, Shigeo Kawata, Ken Uchibori and Takahiro Karino	\\
		\vspace{10truept}
		Utsunomiya University	\\
		Graduate School, 
		Yohtoh 7-1-2, Utsunomiya 321-8585, Japan. mc196858@cc.utsunomiya-u.ac.jp, kwt@cc.utsunomiya-u.ac.jp
	\end{center}
%\end{document}
